6G RIS-aided Single-LEO Localization with Slow and Fast Doppler Effects

6G networks aim to enable applications like autonomous driving by providing complementary localization services through key technologies such as non-terrestrial networks (NTNs) with low Earth orbit (LEO) satellites and reconfigurable intelligent surfaces (RIS). Prior research in 6G localization using single LEO, multi-LEO, and multi-LEO multi-RIS setups has limitations: single LEO lacks the required accuracy, while multi-LEO/RIS setups demand many visible satellites and RISs, which is not always feasible in practice. This paper explores the novel problem of localization with a single LEO satellite and a single RIS, bridging these research areas. We present a comprehensive signal model accounting for user carrier frequency offset (CFO), clock bias, and fast and slow Doppler effects. Additionally, we derive a low-complexity estimator that achieves theoretical bounds at high signal-to-noise ratios (SNR). Our results demonstrate the feasibility and accuracy of RIS-aided single-LEO localization in 6G networks and highlight potential research directions.

==> Figures/TikzFig.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}
[scale=1\columnwidth/10cm,font=\footnotesize]
\begin{axis}[%
width=5cm,
height=2.5cm,
at={(0cm, 9cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.0001,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Sat delay estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	0.156432104780505\\
29.7962839992626	0.0494681750280515\\
39.7962839992626	0.0156432104780518\\
49.7962839992626	0.00494681750280548\\
59.7962839992626	0.00156432104780509\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	2271.1326771386\\
29.7962839992626	0.0515377546471275\\
39.7962839992626	0.0181139734465962\\
49.7962839992626	0.00779926261821184\\
59.7962839992626	0.00552702409760222\\
};
\end{axis}


\begin{axis}[%
width=5cm,
height=2.5cm,
at={(0cm, 4.5cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.00749507041445318,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={RIS delay estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	0.749507041445312\\
29.7962839992626	0.237014937330142\\
39.7962839992626	0.0749507041445331\\
49.7962839992626	0.0237014937330144\\
59.7962839992626	0.00749507041445318\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	3013.6930375954\\
29.7962839992626	3032.43470426451\\
39.7962839992626	0.0631719145974557\\
49.7962839992626	0.0228482468841607\\
59.7962839992626	0.0100127833319976\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(7cm, 9cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.00777984569226848,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m/s]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Sat Doppler estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	0.777984569226829\\
29.7962839992626	0.246020322322176\\
39.7962839992626	0.0777984569226887\\
49.7962839992626	0.024602032232219\\
59.7962839992626	0.00777984569226848\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	1286.17121544512\\
29.7962839992626	0.241926547815047\\
39.7962839992626	0.0803730383671794\\
49.7962839992626	0.0276971928051582\\
59.7962839992626	0.0125743786942445\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(7cm, 4.5cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.01,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m/s]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={RIS Doppler estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	3.79548493890607\\
29.7962839992626	1.20023772318082\\
39.7962839992626	0.379548493890611\\
49.7962839992626	0.120023772318083\\
59.7962839992626	0.0379548493890607\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	1286.13388401456\\
29.7962839992626	0.256138457357912\\
39.7962839992626	0.118934277407562\\
49.7962839992626	0.0856841441041134\\
59.7962839992626	0.0820160106748286\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(14cm, 9cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
% ymin=0.0821235156305157,
ymin = 0.01,
ymax=100,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [deg]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={AOD-H estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	8.21235156305157\\
29.7962839992626	2.59697358852869\\
39.7962839992626	0.821235156305157\\
49.7962839992626	0.259697358852869\\
59.7962839992626	0.0821235156305157\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	36.8450565684234\\
29.7962839992626	38.0173562557511\\
39.7962839992626	0.925101976248053\\
49.7962839992626	0.26925568688826\\
59.7962839992626	0.0981726973804284\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(14cm, 4.5cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
% ymin=0.1,
ymin = 0.01,
ymax=100,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [deg]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={AOD-V estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	13.9736440016682\\
29.7962839992626	4.41885422576212\\
39.7962839992626	1.39736440016682\\
49.7962839992626	0.441885422576213\\
59.7962839992626	0.139736440016682\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	37.0829613740674\\
29.7962839992626	36.0227279369357\\
39.7962839992626	1.57682601526139\\
49.7962839992626	0.531336854805123\\
59.7962839992626	0.144564759404224\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(0cm, 0cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.01,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Position estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	4.10540990005461\\
29.7962839992626	1.29824460127775\\
39.7962839992626	0.410540990005566\\
49.7962839992626	0.129824460127762\\
59.7962839992626	0.041054099000541\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	4646.5026957413\\
29.7962839992626	4269.29434113927\\
39.7962839992626	0.459484856865247\\
49.7962839992626	0.154941333731462\\
59.7962839992626	0.0427917742393268\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(7cm, 0cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.00741084179290927,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Time bias estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	3.11923291434699\\
29.7962839992626	0.986388056190192\\
39.7962839992626	0.311923291434782\\
49.7962839992626	0.0986388056190088\\
59.7962839992626	0.0311923291434657\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	3218.94534142675\\
29.7962839992626	2324.90962773519\\
39.7962839992626	0.255472898804338\\
49.7962839992626	0.119053776308108\\
59.7962839992626	0.0332648301092963\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(14cm, 0cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.00775096741026311,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m/s]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={CFO estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	0.775096741026292\\
29.7962839992626	0.245107110861679\\
39.7962839992626	0.0775096741026352\\
49.7962839992626	0.0245107110861693\\
59.7962839992626	0.00775096741026311\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	1289.41355085786\\
29.7962839992626	25.8442912781656\\
39.7962839992626	0.0803446814292852\\
49.7962839992626	0.0278658259204311\\
59.7962839992626	0.0125856106853796\\
};
\end{axis}

% \begin{axis}[%
% width=26.667in,
% height=15in,
% at={(0in,0in)},
% scale only axis,
% xmin=0,
% xmax=1,
% ymin=0,
% ymax=1,
% axis line style={draw=none},
% ticks=none,
% axis x line*=bottom,
% axis y line*=left
% ]
% \end{axis}
\end{tikzpicture}%

==> Figures/TikzFig2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}
[scale=1\columnwidth/10cm,font=\footnotesize]
\begin{axis}[%
width=5cm,
height=2.5cm,
at={(0cm, 9cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.0001,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Sat delay estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	0.156432104780505\\
24.7962839992626	0.0879682371045935\\
29.7962839992626	0.0494681750280515\\
34.7962839992626	0.0278179991000225\\
39.7962839992626	0.0156432104780518\\
44.7962839992626	0.00879682371045902\\
49.7962839992626	0.00494681750280548\\
54.7962839992626	0.0027817999100025\\
59.7962839992626	0.00156432104780509\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	2391.5398044693\\
24.7962839992626	0.0852940000579745\\
29.7962839992626	0.0496030279774495\\
34.7962839992626	0.0274733887707998\\
39.7962839992626	0.0152024986222784\\
44.7962839992626	0.0102628175025101\\
49.7962839992626	0.00773822716517529\\
54.7962839992626	0.00639913962170057\\
59.7962839992626	0.00560384794488627\\
};
\end{axis}


\begin{axis}[%
width=5cm,
height=2.5cm,
at={(0cm, 4.5cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.00749507041445318,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={RIS delay estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	0.749507041445312\\
24.7962839992626	0.421478782925862\\
29.7962839992626	0.237014937330142\\
34.7962839992626	0.13328329394814\\
39.7962839992626	0.0749507041445331\\
44.7962839992626	0.0421478782925862\\
49.7962839992626	0.0237014937330144\\
54.7962839992626	0.0133283293948142\\
59.7962839992626	0.00749507041445318\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	2752.90710475777\\
24.7962839992626	3145.29282683876\\
29.7962839992626	2943.63360781862\\
34.7962839992626	685.673571177192\\
39.7962839992626	0.0740012894824578\\
44.7962839992626	0.0428481706611463\\
49.7962839992626	0.0215660816726533\\
54.7962839992626	0.0150869817918764\\
59.7962839992626	0.00970881022451034\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(7cm, 9cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.00777984569226848,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m/s]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Sat Doppler estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	0.777984569226829\\
24.7962839992626	0.437492873636699\\
29.7962839992626	0.246020322322176\\
34.7962839992626	0.13834739407841\\
39.7962839992626	0.0777984569226887\\
44.7962839992626	0.0437492873636684\\
49.7962839992626	0.024602032232219\\
54.7962839992626	0.0138347394078419\\
59.7962839992626	0.00777984569226848\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	1259.57821874309\\
24.7962839992626	0.357648426260504\\
29.7962839992626	0.243217204498249\\
34.7962839992626	0.147084298128108\\
39.7962839992626	0.0793372950933824\\
44.7962839992626	0.0488201152808704\\
49.7962839992626	0.0238386716537473\\
54.7962839992626	0.0151816418276013\\
59.7962839992626	0.0105840639689237\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(7cm, 4.5cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.01,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m/s]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={RIS Doppler estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	3.79548493890607\\
24.7962839992626	2.13435803028445\\
29.7962839992626	1.20023772318082\\
34.7962839992626	0.674943271796953\\
39.7962839992626	0.379548493890611\\
44.7962839992626	0.213435803028445\\
49.7962839992626	0.120023772318083\\
54.7962839992626	0.0674943271796953\\
59.7962839992626	0.0379548493890607\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	1259.54490318822\\
24.7962839992626	0.368293864297574\\
29.7962839992626	0.261909928818744\\
34.7962839992626	0.162916941101658\\
39.7962839992626	0.103054012965931\\
44.7962839992626	0.0892523855640574\\
49.7962839992626	0.0846032357036734\\
54.7962839992626	0.0805637795792162\\
59.7962839992626	0.0796968470524272\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(14cm, 9cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
% ymin=0.0821235156305157,
ymin = 0.01,
ymax=100,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [deg]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={AOD-H estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	8.21235156305157\\
24.7962839992626	4.61814466089546\\
29.7962839992626	2.59697358852869\\
34.7962839992626	1.46038556925756\\
39.7962839992626	0.821235156305157\\
44.7962839992626	0.461814466089546\\
49.7962839992626	0.259697358852869\\
54.7962839992626	0.146038556925756\\
59.7962839992626	0.0821235156305157\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	36.5739167733837\\
24.7962839992626	38.354032826079\\
29.7962839992626	38.5564532465156\\
34.7962839992626	10.4186279444425\\
39.7962839992626	0.947164310909001\\
44.7962839992626	0.550615196945047\\
49.7962839992626	0.316617806869229\\
54.7962839992626	0.169479732748226\\
59.7962839992626	0.104771644193285\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(14cm, 4.5cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
% ymin=0.1,
ymin = 0.01,
ymax=100,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [deg]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={AOD-V estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	13.9736440016682\\
24.7962839992626	7.85795748563628\\
29.7962839992626	4.41885422576212\\
34.7962839992626	2.48490434113805\\
39.7962839992626	1.39736440016682\\
44.7962839992626	0.785795748563627\\
49.7962839992626	0.441885422576213\\
54.7962839992626	0.248490434113805\\
59.7962839992626	0.139736440016682\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	36.3488198307436\\
24.7962839992626	32.2251563407421\\
29.7962839992626	33.3493888797708\\
34.7962839992626	15.1515549763775\\
39.7962839992626	4.11109787008343\\
44.7962839992626	0.907376488456943\\
49.7962839992626	0.511978724101239\\
54.7962839992626	0.290191706499346\\
59.7962839992626	0.170868109567974\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(0cm, 0cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.01,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Position estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	4.10540990005461\\
24.7962839992626	2.30864164364646\\
29.7962839992626	1.29824460127775\\
34.7962839992626	0.730056589503743\\
39.7962839992626	0.410540990005566\\
44.7962839992626	0.23086416436464\\
49.7962839992626	0.129824460127762\\
54.7962839992626	0.0730056589503853\\
59.7962839992626	0.041054099000541\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	5017.57242722208\\
24.7962839992626	4972.52598921177\\
29.7962839992626	4232.43415441447\\
34.7962839992626	550.160633106673\\
39.7962839992626	0.798757554288937\\
44.7962839992626	0.266560083613717\\
49.7962839992626	0.144963231148264\\
54.7962839992626	0.0831657029546964\\
59.7962839992626	0.0482124966108023\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(7cm, 0cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.00741084179290927,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Time bias estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	3.11923291434699\\
24.7962839992626	1.75407357063137\\
29.7962839992626	0.986388056190192\\
34.7962839992626	0.554686766669923\\
39.7962839992626	0.311923291434782\\
44.7962839992626	0.175407357063133\\
49.7962839992626	0.0986388056190088\\
54.7962839992626	0.0554686766670014\\
59.7962839992626	0.0311923291434657\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	3907.17544269117\\
24.7962839992626	2699.2856670978\\
29.7962839992626	2208.64857092332\\
34.7962839992626	239.932661698284\\
39.7962839992626	0.523172800551839\\
44.7962839992626	0.18892154979316\\
49.7962839992626	0.113241482410921\\
54.7962839992626	0.0652673753464647\\
59.7962839992626	0.0376869922368128\\
};
\end{axis}

\begin{axis}[%
width=5cm,
height=2.5cm,
at={(14cm, 0cm)},
scale only axis,
xmin=15,
xmax=60,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.00775096741026311,
ymax=10000,
yminorticks=true,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Error [m/s]},
axis background/.style={fill=white},
title style={font=\bfseries},
title={CFO estimation performance},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	0.775096741026292\\
24.7962839992626	0.435868928499486\\
29.7962839992626	0.245107110861679\\
34.7962839992626	0.137833857535535\\
39.7962839992626	0.0775096741026352\\
44.7962839992626	0.0435868928499472\\
49.7962839992626	0.0245107110861693\\
54.7962839992626	0.0137833857535544\\
59.7962839992626	0.00775096741026311\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
19.7962839992626	1260.98297824345\\
24.7962839992626	29.8522202386815\\
29.7962839992626	25.926517745417\\
34.7962839992626	3.41283714338214\\
39.7962839992626	0.0796786893007178\\
44.7962839992626	0.0489114799672099\\
49.7962839992626	0.0238222387594037\\
54.7962839992626	0.0151805162484289\\
59.7962839992626	0.0105689425894322\\
};
\end{axis}

% \begin{axis}[%
% width=26.667in,
% height=15in,
% at={(0in,0in)},
% scale only axis,
% xmin=0,
% xmax=1,
% ymin=0,
% ymax=1,
% axis line style={draw=none},
% ticks=none,
% axis x line*=bottom,
% axis y line*=left
% ]
% \end{axis}
\end{tikzpicture}%
